ReadNet: A Hierarchical Transformer Framework for Web Article Readability Analysis

Analyzing the readability of articles has been an important sociolinguistic task. Addressing this task is necessary to the automatic recommendation of appropriate articles to readers with different comprehension abilities, and it further benefits education systems, web information systems, and digital libraries. Current methods for assessing readability employ empirical measures or statistical learning techniques that are limited by their ability to characterize complex patterns such as article structures and semantic meanings of sentences. In this paper, we propose a new and comprehensive framework which uses a hierarchical self-attention model to analyze document readability. In this model, measurements of sentence-level difficulty are captured along with the semantic meanings of each sentence. Additionally, the sentence-level features are incorporated to characterize the overall readability of an article with consideration of article structures. We evaluate our proposed approach on three widely-used benchmark datasets against several strong baseline approaches. Experimental results show that our proposed method achieves the state-of-the-art performance on estimating the readability for various web articles and literature.

==> tblEmbed.tex <==
\begin{table}
\setlength\tabcolsep{1pt}
\centering
%\vspace{-1em}
%\small
\begin{tabular}{c|ccc|ccc|ccc}

Models&\multicolumn{3}{c|}{{HATT}}&\multicolumn{3}{c|}{{HATT+}}&\multicolumn{3}{c}{ReadNet}\\
\hline

Embeddings&1D&S-G&R-S-G&1D&S-G&R-S-G&1D&S-G&R-S-G\\
\hline
Wiki (\%)& 86.52  & 87.71& 89.24 &  88.43 & 89.87& 90.83 &90.31 &91.38&\textbf{92.71}\\
CEE (\%)&46.03 &51.21&52.51& 51.27 &51.32& 52.14 &51.82 &52.82 &\textbf{54.42}\\
Weebit (\%)&87.25 &88.43&89.37 & 89.28 &90.24& 91.37 &90.81 &91.71&\textbf{92.51}\\
\hline
\end{tabular}
\caption{Accuracy of readability analysis using different models and word embeddings. Embedding methods are readability score (1D) defined by Equation~\ref{eq:diff}, original Skip-Gram (S-G) and our proposed readability-aware Skip-Gram (R-S-G). Models include HATT, HATT with explicit features (HATT+) and our proposed ReadNet.}
\label{tbl:word}

\end{table}


==> transfer.tex <==
\section{Transfer Learning}

The goal of transfer learning is to use labeled data from related tasks to make the current task easier. We adopt the sitting of asymmetric transfer:

Given a large amount of supervised data for a set of related tasks, the goal is to improve prediction quality on a target task which training data is scarce.

Readability evaluation problem suffers from the lack of well-labeled data. Traditional benchmark dataset which is labeled by domain experts only contains a small number of articles. For instance, Cambridge English Exam contains 800 articles and Weebit contains around 8 thousands articles. It is time and resource expensive to hire domain experts to label more data. On the other hand, with the emerging of online encyclopedia applications such as Wikipedia, it provides a huge amount of training dataset. For instance, English Wikipedia and Simple-English Wikipedia contain more than 100 thousands articles which can be used to train a deep learning model.

==> word.tex <==
 \subsection{Word Representations}

%We hereby introduce our word readability representation.
In this subsection, we first present an effective word embedding technique to indicate word difficulty.

\subsubsection{Difficulty Measurement of Words}
As shown in research~\cite{coxhead2000new,Lexicon},  words with higher frequency in the literature often appear to be easier. The ranking of words based on frequency can be considered as the reverse ranking of difficulty. For instance, using Wikipedia-based dataset~\cite{wikidata} in our training, the top-ranked words are stop words such as ``in", ``a", ``is". While those low ranked words often consists of difficult ones such as ``marionette" ``depigmentation".

Assume the corpus has $N$ words. Each word $w$ is ranked by the frequency in descending order with the ranking $rank(w)$. We define a difficulty score for word $w$ with Equation~\ref{eq:diff}. In this function, a $\log$ function in the numerator is adopted to scale the measure of difficulty. Words with lower ranks are expected to show less variation in difficulty. The $\log(N)$ in the denominator is used to normalize the word difficulty score to the range of [0, 1].
\begin{equation}\label{eq:diff}
d(w) =\frac{ \log(rank(w))} { \log(N)}
\end{equation}


\subsubsection{Word Embeddings for Readability}
Word embedding techniques play an important role in transforming discrete words from a large corpus into a continuous vector based on their context, hence are the essential feature maps for neural document models.
\paragraph{Skip-Gram model}
Existing word embedding approaches aim to capture semantic similarity of words based on their context similarity, and simulate such similarity in the form of vector inner product.
The skip-gram model~\cite{word2vec} is one of the most used word embedding approaches which aims to predict the target word given its context words within a sliding window.

For a sequence of words $ T = \{w_1,..., w_M\}$, the skip-gram model is trained by maximizing the conditional log-likelihood of a word over its context words, which is defined as below:

\begin{equation}
L(T) = \frac{1}{T} \sum_{t=1}^{T} \sum_{ -c \leq j \leq c } \log p(w_{t+j}| w_t)
\end{equation}

In the above equation, the sliding window size is $2c+1$. The conditional probability  $p(w_{t+j}| w_t)$ is a softmax function defined in Equation~\ref{condition} where ${v_w}$ and  ${v'_w}$ as ``input" and ``output" vector representations of $w$.

\begin{equation}\label{condition}
p(w_O|w_I) = \frac{exp({{v}'_{w_O}} ^\intercal {v}_{w_I})}{\sum_{w \in W} exp({{v'}_{w}}^\intercal  {v}_{w_I})}.
\end{equation}


\paragraph{Readability-aware Skip-Gram model}
the skip-gram model have been extended to support different applications such as topic-aware embeddings~\cite{topicalEmbed,topicalEmbed2}. However, our task requires to encode the word difficulty information into the word representations which has not been resolved by previous works.
For a toy example, three sentences ``a nice cat", ``a pretty cat" and ``a gorgeous cat". Simply adopting Skip-Gram model directly obtains very similar embedded vectors for the three words ``nice", ``pretty" and ``gorgeous". If the difficulty information is involved in word embeddings, ``nice" and ``pretty" should be considered closer than ``nice" and ``gorgeous", since ``gorgeous" is a relatively complicated word.

In this case, we adapt the conditional log likelihood of Skip-Gram as the following

\begin{equation}
p(w_O|w_I) = \frac{exp(({{v}_{w_O}'} ^\intercal {v}_{w_I})^{D(w_O, w_I)})}{\sum_{w \in W} exp(({{v}_{w}'}^\intercal  {v}_{w_I})^{D(w, w_I)})}.
\end{equation}

\noindent
where $D(w_O, w_I)$ is a function to indicate the similarity of difficulty between these two words $w_O$ and $w_I$. As we have stated that there is {highly negative correlation between difficulty and word frequency}, we adopt Equation~\ref{eq:diff} to estimate the word difficulty as $d(w_O)$ and $d(w_I)$. $D(w_O, w_I)$ is defined as follows.
$D(w_O, w_I) = |d(w_O) - d(w_I) | + 1$.

Since it is impossible to enumerate all $w$, we adopt negative sampling for efficient approximiation. The Noise Contrastive Estimation (NCE) technique~\cite{NCE} is used to obtain a computationally efficient term of the softmax log likelihood
\begin{align*}
\log p(w_O|w_I) =	D(w_O, w_I) \log \sigma({{v}_{w_O}'} ^\intercal {v}_{w_I} ) \\
+ \sum_{i=1}^{k} E_{w_i \sim P_n(w)}[D(w_i, w_I)  \log \sigma({ - {v}_{w_i}'} ^\intercal {v}_{w_I} )]
\end{align*}
for which $P_n(w)$ is the distribution of words. The goal is to distinguish the target word $w_O$ and a random word $w_i$.


